The Center of Attention: Center-Keypoint Grouping via Attention for Multi-Person Pose Estimation

We introduce CenterGroup, an attention-based framework to estimate human poses from a set of identity-agnostic keypoints and person center predictions in an image. Our approach uses a transformer to obtain context-aware embeddings for all detected keypoints and centers and then applies multi-head attention to directly group joints into their corresponding person centers. While most bottom-up methods rely on non-learnable clustering at inference, CenterGroup uses a fully differentiable attention mechanism that we train end-to-end together with our keypoint detector. As a result, our method obtains state-of-the-art performance with up to 2.5x faster inference time than competing bottom-up methods. Our code is available at https://github.com/dvl-tum/center-group .

==> LaTeX/tables/ablation/formulation.tex <==
\usepackage{booktabs}
\newcommand{\ra}[1]{\renewcommand{\arraystretch}{#1}}
\begin{table*}\centering
\ra{1.3}
\begin{tabular}{@{}rrrrcrrrcrrr@{}}\toprule
& \multicolumn{3}{c}{$w = 8$} & \phantom{abc}& \multicolumn{3}{c}{$w = 16$} &
\phantom{abc} & \multicolumn{3}{c}{$w = 32$}\\
\cmidrule{2-4} \cmidrule{6-8} \cmidrule{10-12}
& $t=0$ & $t=1$ & $t=2$ && $t=0$ & $t=1$ & $t=2$ && $t=0$ & $t=1$ & $t=2$\\ \midrule
$dir=1$\\
$c$ & 0.0790 & 0.1692 & 0.2945 && 0.3670 & 0.7187 & 3.1815 && -1.0032 & -1.7104 & -21.7969\\
$c$ & -0.8651& 50.0476& 5.9384&& -9.0714& 297.0923& 46.2143&& 4.3590& 34.5809& 76.9167\\
$c$ & 124.2756& -50.9612& -14.2721&& 128.2265& -630.5455& -381.0930&& -121.0518& -137.1210& -220.2500\\
$dir=0$\\
$c$ & 0.0357& 1.2473& 0.2119&& 0.3593& -0.2755& 2.1764&& -1.2998& -3.8202& -1.2784\\
$c$ & -17.9048& -37.1111& 8.8591&& -30.7381& -9.5952& -3.0000&& -11.1631& -5.7108& -15.6728\\
$c$ & 105.5518& 232.1160& -94.7351&& 100.2497& 141.2778& -259.7326&& 52.5745& 10.1098& -140.2130\\
\bottomrule
\end{tabular}
\caption{Caption}
\end{table*}

==> LaTeX/tables/benchmark/ochuman.tex <==
%%%%%%%%%%%%%%%%%%%%%%
% Evalution OCHumans validation and test split
%%%%%%%%%%%%%%%%%%%%%%
\begin{table}
\begin{center}
\resizebox{\columnwidth}{!}{
\begin{tabular}{l|l|c|c}
\hline
Method & Backbone & Val & Test \\
\hline
\multicolumn{4}{c}{Top-down methods} \\
\hline
RMPE  & Hourglass & 38.8 & 30.7\\
SBL & ResNet50 & 37.8 & 30.4 \\
SBL & ResNet152 & 41.0 & 33.3 \\
\hline
\multicolumn{4}{c}{Bottom-up methods} \\
\hline
AE\textsuperscript{+} & Hourglass       & 40.0 & 32.8 \\
AE & HrHRNet-W48 \cite{hrnet}  & 40.9  &  40.3\\
AE\textsuperscript{+} \cite{hrnet} & HrHRNet-W48 & 43.0  & 41.9 \\
HGG \cite{hgg}                  & Hourglass       & 35.6 & 34.8 \\
HGG\textsuperscript{+} \cite{hgg}& Hourglass       & 41.8 & 36.0 \\

Ours                  & HrHrNet-W48 & 42.0 & 4 \\ 
Ours \textsuperscript{+} & HrHrNet-W48 & 43.2 & \textcolor{red}{TODO} \\
\hline
\end{tabular}
}
\end{center}
\caption{\gui{Reestructure this table. We shouldn't mix grouping with method}}
\end{table}
